That is a Known Lie: Detecting Previously Fact-Checked Claims

The recent proliferation of "fake news" has triggered a number of responses, most notably the emergence of several manual fact-checking initiatives. As a result and over time, a large number of fact-checked claims have been accumulated, which increases the likelihood that a new claim in social media or a new statement by a politician might have already been fact-checked by some trusted fact-checking organization, as viral claims often come back after a while in social media, and politicians like to repeat their favorite statements, true or false, over and over again. As manual fact-checking is very time-consuming (and fully automatic fact-checking has credibility issues), it is important to try to save this effort and to avoid wasting time on claims that have already been fact-checked. Interestingly, despite the importance of the task, it has been largely ignored by the research community so far. Here, we aim to bridge this gap. In particular, we formulate the task and we discuss how it relates to, but also differs from, previous work. We further create a specialized dataset, which we release to the research community. Finally, we present learning-to-rank experiments that demonstrate sizable improvements over state-of-the-art retrieval and textual similarity approaches.

==> results-table-original.tex <==

\begin{table*}[tbh]
    \small
    \centering
    \begin{tabular}{@{}l@{}c*{12}c@{}}
        \toprule
        \bf Experiment & \multicolumn{1}{c}{\bf MRR} & \multicolumn{6}{c}{\bf MAP@$k$} & \multicolumn{6}{c}{\bf HasPositives@$k$} \\
        \cmidrule(lr){3-8}\cmidrule(lr){9-14}
        {} & {} & 1 & 3 & 5 & 10 & 20 & all & 1 & 3 & 5 & 10 & 20 & 50 \\
        \midrule 
        \multicolumn{14}{c}{\bf IR (BM25; full database)}\\
        \midrule 
        IR:Title	&	.288	&	.216	&	.259	&	.261	&	.268	&	.272	&	.276	&	.220	&	.330	&	.346	&	.401	&	.464	&	.535 \\
        IR:\verclaim	&	.435	&	.366	&	.404	&	.413	&	.415	&	.419	&	.422	&	.378	&	.472	&	.511	&	.527	&	.574	&	.629 \\
        IR:Body	&	\bf.565	&	\bf.484	&	\bf.538	&	\bf.546	&	\bf.552	&	\bf.556	&	\bf.560	&	\bf.488	&	\bf.614	&	\bf.653	&	\bf.700	&	\bf.740	&	\bf.811 \\
        IR:Title+\verclaim+Body	&.526	&	.425	&	.504	&	.507	&	.513	&	.516	&	.519	&	.433	&	\bf.614	&	.630	&	.661	&	.717	&	.772 \\
        \midrule 
        \multicolumn{14}{c}{\bf Semantic Matching - BERT \& co. (matching against \verclaim~only; full database)}\\
        \midrule
        BERT:base,uncased	&	.268	&	.204	&	.242	&	.251	&	.259	&	.260	&	.264	&	.204	&	.299	&	.338	&	.393	&	.409	&	.496 \\
		RoBERTa:base	&	.209	&	.173	&	.194	&	.198	&	.203	&	.205	&	.207	&	.173	&	.220	&	.236	&	.283	&	.315	&	.346 \\
		sentence-BERT:base	&	.377	&	.311	&	.352	&	.354	&	.361	&	.366	&	.370	&	.315	&	\bf.417	&	\bf.425	&	\bf.480	&	\bf.551	&	\bf.614 \\
		sentence-BERT:large	&	\bf.395	&	\bf.354	&	\bf.367	&	\bf.372	&	\bf.381	&	\bf.382	&	\bf.386	&	\bf.362	&	.393	&	.417	&	\bf.480	&	.496	&	.582 \\
        \midrule 
        \multicolumn{14}{c}{\bf BERT on Full Articles (sentence-BERT:large matching against \verclaim~+ Title + top-$n$ article body sentences; full database)}\\
        \midrule        
        sentence-BERT: n = 3	&	.515	&	\bf.441	&	.478	&	.493	&	.498	&	.501	&	.505	&	\bf.457	&	.528	&	\bf.598	&	\bf.638	&	\bf.693    &    \bf.756 \\
        sentence-BERT: n = 4	&	\bf.517	&	\bf.441	&	\bf.487	&	\bf.497	&	\bf.500	&	\bf.505	&	\bf.508	&	\bf.457	&	\bf.551	&	\bf.598	&	.622	&	.685    &   \bf.756 \\
        sentence-BERT: n = 5	&	.515	&	.433	&	.484	&	.491	&	.498	&	.502	&	.505	&	.449	&	\bf.551	&	.583	&	\bf.638	&	.685    &    .748 \\
        sentence-BERT: n = 6	&	.509	&	.429	&	.480	&	.485	&	.491	&	.497	&	.500	&	.441	&	.543	&	.567	&	.614	&	\bf.693    &    .740 \\
        \midrule 
        \multicolumn{14}{c}{\bf Reranking (IR \& sentence-BERT:large matching against \verclaim~+ Title + top-4 article body sentences; top-$N$ from IR)}\\
        \midrule        
        Rerank-IR-top-10	&	.586	&	.528	&	.572	&	.578	&	.583	&	---	&	---	&	.512	&	.638	&	.693	&	.701	&	---	&	--- \\
        Rerank-IR-top-20	&	.586	&	.521	&	.572	&	.577	&	.580	&	.583	&	---	&	.512	&	.646	&	.685	&	.709	&	.740	&	--- \\
        Rerank-IR-top-50	&	.600	&	.519	&	.568	&	.584	&	.590	&	.590	&	.594	&	.520	&	.638	&	\bf.717	&	\bf.772	&	.780	&	.811 \\
        Rerank-IR-top-100	&	\bf.608	&	\bf.531	&	\bf.580	&	\bf.588	&	\bf.597	&	\bf.599	&	\bf.602	&	\bf.535	&	\bf.654	&	.685	&	.740	&	\bf.787	&	\bf.819 \\
        Rerank-IR-top-200	&	.605	&	.529	&	.575	&	.585	&	.594	&	.598	&	.599	&	\bf.535	&	.646	&	.685	&	.756	&	.803	&	.811 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{PolitiFact:} evaluation results on the test set.}
    \label{table:results-politifact}
\end{table*}


\begin{table*}[tbh]
    \small
    \centering
    \begin{tabular}{@{}l@{}c*{12}c@{}}
        \toprule
        \bf Experiment & \multicolumn{1}{c}{\bf MRR} & \multicolumn{6}{c}{\bf MAP@$k$} & \multicolumn{6}{c}{\bf HasPositives@$k$} \\
        \cmidrule(lr){3-8}\cmidrule(lr){9-14}
        {} & {} & 1 & 3 & 5 & 10 & 20 & all & 1 & 3 & 5 & 10 & 20 & 50 \\
        \midrule 
        \multicolumn{14}{c}{\bf IR (BM25; full database)}\\
        \midrule 
         IR:Title       &  .619  &  .538  &  .573  &  .583  &  .587  &  .590  &  .592  &  .538  &  .673  &  .724  &  .759  &  .804  &  .844  \\
        IR:\verclaim  &  .655  & \bf .555 & .589 & .598 & .600 & .602 & .605 & \bf .558 & .729 & .769 & .784 & .809 & .864 \\
        IR:\verclaim+Title  &  \bf .664  & \bf .555 & \bf .592 & \bf .600 & \bf .605 & \bf .608 & \bf .609 & \bf .558 & \bf .739 & \bf .774 & \bf .814 & \bf.849 & \bf .879  \\
        \midrule 
        \multicolumn{14}{c}{\bf Semantic Matching - BERT \& co. (matching against \verclaim~only; full database)}\\
        \midrule
        sentence-BERT-base:Title  & .474  & .397 & .417 & .425 & .430 & .434 & .437 & .397 & .528 & .563 & .598 & .658 & .729  \\
        sentence-BERT-base:\verclaim  & .515  & .402 & .489 & .504 & .510 & .512 & .515 & .402 & .593 & \bf .653 & \bf .698 & \bf .739 & .784  \\
        sentence-BERT-large:\verclaim  & \bf .543 & \bf .457 & \bf .518 & \bf .527 & \bf .533 & \bf .535 & \bf .538 & \bf .457 & \bf .603 & .648 & .693 & .724 & \bf .794  \\
        \midrule 
        \multicolumn{14}{c}{\bf Reranking (IR \& sentence-BERT:large matching against \verclaim~+ Title; top-$N$ from IR)}\\
        \midrule
        Rerank-IR-top-10  & .764 & .687 & .762 & .764 & .764 & --- & --- & .673 & .859 & .869 & .869 & --- & --- \\
        Rerank-IR-top-20  & .781 & .686 & .773 & .780 & .781 & .781 & --- & .678 & .869 & \bf .905 & \bf .920 & .920 & --- \\
        Rerank-IR-top-50  & \bf .788 & \bf .691 & \bf .780 & \bf .782 & \bf .784 & \bf .784 & \bf .787 & \bf .693 & \bf .874 & .894 & .915 & .925 & .930 \\
        Rerank-IR-top-100  & .775 & .669 & .758 & .760 & .760 & .760 & .774 & .673 & .859 & .889 & .910 & .925 & .930 \\        
        Rerank-IR-top-200 & .778 & .672 & .762 & .764 & .764 & .764 & .777 & .678 & .864 & .884 & .910 & \bf .930 & \bf .950 \\        
        \bottomrule 
    \end{tabular}
    \caption{\textbf{Snopes:} evaluation results on the test set.}
    \label{table:snopes-results}
\end{table*}


==> snopes.tex <==
\begin{table*}[tbh]
    \small
    \centering
    \begin{tabular}{@{}l@{}c*{12}c@{}}
        \toprule
        \bf Experiment & \multicolumn{1}{c}{\bf MRR} & \multicolumn{6}{c}{\bf MAP@$k$} & \multicolumn{6}{c}{\bf HasPositives@$k$} \\
        \cmidrule(lr){3-8}\cmidrule(lr){9-14}
        {} & {} & 1 & 3 & 5 & 10 & 20 & all & 1 & 3 & 5 & 10 & 20 & 50 \\
        \midrule 
        \multicolumn{14}{c}{\bf IR (BM25; full database)}\\
        \midrule 
        IR:Title       &  .619  &  .538  &  .573  &  .583  &  .587  &  .590  &  .592  &  .538  &  .673  &  .724  &  .759  &  .804  &  \bf .844  \\
        IR5:NormClaim  &  .892  &  .835  &  .885  &  .892  &  .892  &  .892  &  .892  &  .840  &  \bf .940  & \bf .970  &  .970  &  .970  &  .970  \\
        IR:NormClaim+Title  &  \bf .928  &  \bf .895  &  \bf .910  & \bf .917  & \bf .918  & \bf .918  & \bf .919  & \bf .900  &  \bf .940  &  \bf .970  &  \bf .980  &  \bf .980  &  \bf .980  \\
        \midrule 
        \multicolumn{14}{c}{\bf BERT \& co. (sentence-BERT:base)}\\
        \midrule
        sentence-BERT:Title  & \bf .827  & \bf .785  & \bf .818  & \bf .823  & \bf .825  & \bf .826  & \bf .827  & \bf .790  &  \bf .850  &  \bf .870  &  \bf .880  & \bf .900  & \bf .920  \\
        sentence-BERT:NormClaim  &  .823  &  .775  &  .815  &  .817  &  .819  &  .821  &  .823  &  .780  &  \bf .850  &  .860  &  \bf .880  & \bf .900  &  .910  \\
        \midrule 
        \multicolumn{14}{c}{\bf Reranking (IR \& sentence-BERT: matching against NormClaim + Title; top-$N$ from IR)}\\
        \midrule
        Rerank-IR-top-3  &  .913  &  .900  &  .913  &  ---  &  ---  &  ---  &  ---  &  .890  &  .940  & ---  &  ---  &  ---  &  ---  \\
        Rerank-IR-top-5  &  .943  &  .889  &  .904  & \bf .943  &  ---  &  ---  &  ---  & \bf .920  &  .970  & .970  &  ---  &  ---  &  ---  \\
        Rerank-IR-top-10  & \bf .948  & \bf .913  & \bf .936  &  .936  & \bf .948  &  ---  &  ---  & \bf .920  & \bf .980  & \bf .980  & \bf .980  &  ---  &  ---  \\
        Rerank-IR-top-20  & \bf .948  &  .909  &  .934  &  .935  &  .935  & \bf .948  &  ---  & \bf .920  &  .970  & \bf .980  & \bf .980  & \bf .980  &  ---  \\
        Rerank-IR-top-50  & \bf .948  &  .789  &  .789  &  .789  &  .790  &  .791  & \bf .948  & \bf .920  &  .970  & \bf .980  & \bf .980  & \bf .980  & \bf .980  \\
        \bottomrule 
    \end{tabular}
    \caption{Evaluation results on test set of the Snopes dataset.}
    \label{table:snopes-results}
\end{table*}

\section{Experiments on Snopes}
\label{sec:discuss}

We further performed experiments with Snopes, this time focusing on claims from Twitter, that have a corresponding normalized claim, described in Snopes. This is an arguably much easier case, as social media messages are self-contained and easier to isolate compared to claims in speeches and debates, which need more context to understand. 

\paragraph{Data.} The data we have collected from Snopes is comprised of \textit{NormClaim}, \textit{Title}, \textit{TruthValue} and \textit{Claim}. Note that a \textit{NormClaim} can pair with many \textit{Claims}. Here is an easy example:

\begin{itemize}
    \item \textbf{NormClaim:} \emph{Kanye West and Kim Kardashian announced that they were divorcing in October 2018.}
    \item \textbf{Claim:} \emph{Welp\ldots it’s official\ldots Kim Kardashian finally decided to divorce Kanye West… https://t.co/C2p25mxWJO --- Ashlee Marie Preston (@AshleeMPreston) October 12, 2018}
    \item \textbf{Claim:} \emph{Kim Kardashian and Kanye West are splitting up ���� https://t.co/epwKG7aSBg pic.twitter.com/u7qqojWVlR --- ELLE Magazine (US) (@ELLEmagazine) October 18, 2018}
\end{itemize}

And here is hard case:

\begin{itemize}
\item \textbf{NormClaim:} \emph{U.S. Sen. Elizabeth Warren said or argued to the effect that taxpayers must fund sex reassignment surgery.}
\item \textbf{Claim:} \emph{Everyone should be able to access high-quality, affordable, gender-affirming health care. But the Trump administration is trying to roll back important protections for trans Americans. Help fight back by leaving a comment for HHS in protest: https://t.co/pKDcOqbsc7 --- Elizabeth Warren (@ewarren) August 13, 2019}
\end{itemize}

Our Snopes dataset consists of 1000 claims and 788 corresponding normalized claims. We combined our normalized claims with another 10000 extracted from the database of \emph{ClaimsKG}~\cite{ClaimsKG}, which also originate from Snopes. Most of the claims fall into the easy \textit{Type-1} category, as described in \ref{sec:claim-normclaim-pair}. We release this dataset together with the PolitiFact data.\textsuperscript{\ref{footnote:published-dataset-link}}

%TODO: Briefly describe the data, with some examples, but give the examples in the text (one easy, and one hard example? Also, with multiple inputs claims.), not as a table. Say that this time, there are multiple possible original input claims for the same normalized claim. Give some statistics. Say that the data is released on the same URL as the PolitiFact data above.

\paragraph{Experiments.} 
We performed experiments similar to those for PolitiFact, with one major difference --- that we do not use the article body when we perform the matching. This is because in the Snopes page format, the original claims, e.g.,~the tweet from above, would be included in the article body. Thus, matching against the article body would give away the answer.\footnote{Note that the use of debates for PolitiFact above did not cause such issues as the original claim in the debate/speech is not included in the article body verbatim.}

%TODO: Put your table here, following the format for Table 4.  Explain that this time, we cannot compare to the full text. Can you rename your rows to match the same names as in Table 4? Do not worry, if you do not have some of their experiments.

\paragraph{Results.} 
Table~\ref{table:snopes-results} shows the evaluation results. We can see that BM25 is a very strong baseline due to the higher word overlap between the input claims and the normalized claims. Yet, we show that BM25 can easily be improved by re-ranking.

%TODO: Discuss briefly the results: this time, the task is much easier, the baseline is very high. Yet, you manage to improve with the same BM25 + sentence-BERT reranking.


